Communication-Efficient Federated Learning with Accelerated Client Gradient

Federated learning often suffers from slow and unstable convergence due to the heterogeneous characteristics of participating client datasets. Such a tendency is aggravated when the client participation ratio is low since the information collected from the clients has large variations. To address this challenge, we propose a simple but effective federated learning framework, which improves the consistency across clients and facilitates the convergence of the server model. This is achieved by making the server broadcast a global model with a lookahead gradient. This strategy enables the proposed approach to convey the projected global update information to participants effectively without additional client memory and extra communication costs. We also regularize local updates by aligning each client with the overshot global model to reduce bias and improve the stability of our algorithm. We provide the theoretical convergence rate of our algorithm and demonstrate remarkable performance gains in terms of accuracy and communication efficiency compared to the state-of-the-art methods, especially with low client participation rates. The source code is available at our project page.

==> sections/discussion.tex <==
\section{Discussion} 
\label{sec:discussion}
\iffalse
\subsection{Comparision with NAG}
Let $x^t:=\theta^t+\lambda \Delta^t$ and $\nabla (\theta^t) := \theta^{t+1} - x^t$. Then $\Delta^{t+1} = \tau\nabla(\theta^t) + \lambda \Delta^t$. After $t$ communication round we have:


\begin{equation}
\begin{aligned}
x^{t+1}&=\theta^{t+1}+\lambda \Delta^{t+1}
\\&=x^t +\tau\nabla(\theta^t)+\lambda(\tau\nabla(\theta^t) + \lambda \Delta^t)
\\&
=x^t+\tau\nabla(\theta^t) +\tau\underset{i=0}{\overset{t}{\Sigma}}\lambda^{i+1}\nabla(\theta^{t-i})
\end{aligned}
\end{equation}

FedAGM is a federated algorithm. But, if we have N=1 as total client who always participate and do single local update, then we recover the Nesterov Accelerated momentum, which is widely used in centralized learning.
\fi

==> sections/method_before.tex <==
% !TEX root = ../main.tex
\iffalse
%
\setlength{\textfloatsep}{15pt}
\begin{algorithm}[t]
\caption{FedACG}
\label{alg:proposed_method}
\SetAlgoLined
\KwIn{$\beta$, $\lambda$, initial server model $\theta^0$, number of clients $N$, number of local iterations $K$, number of communication rounds $T$, local learning rate $\eta$}
Initialize $m^{0}=0$

 \For{$\text{each round}~t = 1,2, \dots ,T$}{
  Sample subset of clients $S_t \subseteq \{1, \dots, N\}$

Server sends $\theta^{t-1} + \lambda m^{t-1}$ to all clients $i \in S_t$

\For{$\text{each client}~ i \in S_t,~\textbf{in parallel}$}{
%Set $\theta_{i,0}^t=\theta^t-\lambda\Delta^t$
$\theta_{i,0}^t \leftarrow {\theta^{t-1} + \lambda m_{t-1}}$

\For{$k = 1, \dots ,K$}{
%{${\underset{\theta_{i,k}^t}{\operatorname{argmin}}}~ L_i(\theta_{i,k}^t) = \newline
%\hspace*{3.33em} \alpha f_i(\theta_{i,k}^t
%) + \frac{\beta}{2}\|\theta_{i,k}^t-(\theta^t-\lambda\Delta^t)\|^2$  }
%$\mathcal{L}_i(\theta_{i,k-1}^t) \leftarrow {f_i(\theta_{i,k-1}^t) + \frac{\beta}{2}\|\theta_{i,k-1}^t - \theta_{i,0}^t\|^2}$
$f_i(\theta_{i,k-1}^t) \leftarrow {\ell_i(\theta_{i,k-1}^t) + \frac{\beta}{2}\|\theta_{i,k-1}^t - \theta_{i,0}^t\|^2}$

${\theta_{i,k}^t \leftarrow \theta_{i,k-1}^t - \eta \nabla f_i(\theta_{i,k-1}^t) }$
}
$\Delta^t_i =\theta_{i,K}^{t}-(\theta^{t-1} + \lambda m_{t-1})$

Client sends  $\Delta^t_i$
back to the server}
\textbf{In server:}

%\quad $\theta^{t}$ = $\frac{1 }{|S_t|} \Sigma_{i \in S_t}\theta_{i,K}^{t}$
\quad $\Delta^t =\frac{1}{|S_t|}\underset{i \in S_t}{\Sigma}\Delta^t_i$

\quad $\theta^{t} = \theta^{t-1} + \Delta^t$

\quad $m_{t}= \Delta^t + \lambda m_{t-1}$
}
\textbf{Return} ~$\theta^{t}$
\end{algorithm}
\fi 

%
%
\setlength{\textfloatsep}{15pt}
\begin{algorithm}[t]
\caption{FedACG}
\label{alg:proposed_method}
\SetAlgoLined
\KwIn{$\beta$, $\lambda$, initial server model $\theta^0$, number of clients $N$, number of local iterations $K$, number of communication rounds $T$, local learning rate $\eta$}
Initialize $m^{0}=0$

 \For{$\text{each round}~t = 1,2, \dots ,T$}{
  Sample subset of clients $S_t \subseteq \{1, \dots, N\}$

Server sends $\theta^{t-1} + \lambda m^{t-1}$ to all clients $i \in S_t$

\For{$\text{each client}~ i \in S_t,~\textbf{in parallel}$}{
%Set $\theta_{i,0}^t=\theta^t-\lambda\Delta^t$
$\theta_{i,0}^t \leftarrow {\theta^{t-1} + \lambda m^{t-1}}$

\For{$k = 1, \dots ,K$}{
%{${\underset{\theta_{i,k}^t}{\operatorname{argmin}}}~ L_i(\theta_{i,k}^t) = \newline
%\hspace*{3.33em} \alpha f_i(\theta_{i,k}^t
%) + \frac{\beta}{2}\|\theta_{i,k}^t-(\theta^t-\lambda\Delta^t)\|^2$  }
\jkkim{Sample minibatch of data $(x, y) \sim \mathcal{D}_i$}

$f_i(\jkkim{(x,y)};\theta_{i,k-1}^t) \leftarrow {\ell_i(\jkkim{(x,y)};\theta_{i,k-1}^t) + \frac{\beta}{2}\|\theta_{i,k-1}^t - \theta_{i,0}^t\|^2}$
%$f_i(\theta_{i,k-1}^t) \leftarrow {\ell_i(\theta_{i,k-1}^t) + \frac{\beta}{2}\|\theta_{i,k-1}^t - \theta_{i,0}^t\|^2}$

${\theta_{i,k}^t \leftarrow \theta_{i,k-1}^t - \eta \nabla f_i(\theta_{i,k-1}^t) }$
}
Client sends  $\theta_{i,K}^t$
back to the server}
\textbf{In server:}

\quad $\theta^{t}$ = $ \sum_{i \in S_t} \omega_i \theta_{i,K}^{t}$

\quad $m^{t}=\theta^{t}-\theta^{t-1}$
}
\textbf{Return} ~$\theta^{t}$
\end{algorithm}
%

\section{{FedACG}}
%\section{Proposed Method}
\label{sec:method} 
\ghkim{To reduce the inconsistency between the local models and the consequent divergence of the global one, we incorporates the global momentum into local updates for guiding local models.
\cref{alg:proposed_method} presents the procedure of the proposed approach, FedACG.
We also discuss why FedACG is desirable for the real-world federated learning setting.}
%To tackle the aforementioned challenge, we propose FedACG that addresses client heterogeneity. We also discuss why FedACG is desirable for the real-world federated learning setting.
%This section first describes FedACG algorithm and discuss how it solves the problem of client heterogeneity. Then we show that FedACG is desirable for the real-world federated learning settings.


\subsection{{Accelerated client gradient}}

%\paragraph{\revision{[Motivation of the proposed method]}}
%\bhr{\bf To reduce the gap between the local and global objective function, our main idea is to incorporate global gradient information into local updates by accelerating the current model with global momentum.}
\ghkim{The main idea of this paper, accelerated client gradient, is to make clients look ahead the slope of the global loss.}
\jkkim{%by calculating 
To this end, we calculate each client's local gradient not with respect to the previous global model but with respect to the approximated future position of the global parameters.}
\iffalse
To reduce the inconsistency between the local models and the consequent divergence of the global one, we incorporate the global momentum into local updates for guiding local models and accelerating the convergence of the global model.
This subsection describes our main idea of this paper, accelerated client gradient, in detail, and \cref{alg:proposed_method} presents the procedure of the proposed approach, FedACG.
\fi

%cref{alg:proposed_method} presents the pseudocode of the proposed approach, FedACG.
%The main modification in FedAGM compared to FedAvg is that the central server first quantifies the server update direction $\Delta^t$ and broadcasts the accelerated global model $\theta^t - \lambda \Delta^t$ instead of the current global model $\theta$. 
%\ghkim{In each communication round $t \in \{1,\dots,T\}$, the server quantifies the global update momentum $m_t$ by the exponential updates with decay coefficient as $m_t = \Delta^t + \lambda m_{t-1}$, where $\Delta^t$ indicates the expectation of local updates in active client set $S_t \subseteq \{1,\dots,N\}$, \ie $\Delta^t =\underset{i \in S_t}{\Sigma}\frac{|\mathcal{D}_i|}{|\mathcal{D}_{S_t}|}\Delta^t_i$}.
In the $t^\text{th}$ communication round, the server quantifies the server update momentum $m^{t-1} := \theta^{t-1}-\theta^{t-2}$, and broadcasts the accelerated global model $\theta^{t-1} + \lambda m^{t-1}$ to the active client set $\mathcal{S}_{t} \subseteq \{1,\dots,N\}$, where $\lambda \in (0, 1]$ controls the importance of the global momentum.
\ghkim{Each participating client initialize its local model from the momentum-integrated point, \ie $\theta^t_{i, 0} = \theta^{t-1} + \lambda m^{t-1}$, and performs $K$ steps of local updates.}
%Starting with the integrated model as an initial point, \ie $\theta^t_{i, 0} = \theta^{t-1} + \lambda m^{t-1}$, each participating client optimizes a local objective function.
%Each participating client optimizes its local model from the momentum-integrated initialization, \ie $\theta^t_{i, 0} = \theta^{t-1} + \lambda m^{t-1}$.
%{The local objective function is defined as the sum of its local empirical loss function and a penalized loss function which is based on the local online model and the received server model:}
%The objective of each client is the sum of its empirical loss on the local data and a penalty from the difference between the local online model and the accelerated global model, which is given by
%
%$\Delta^t=\theta^{t}-\theta^{t-1}$, and broadcasts the accelerated global model $\theta^t + \lambda \Delta^t ~(0 < \lambda < 1)$ to the currently active client set $S_{t}$.
%Starting with the integrated model as an initial point, \ie $\theta^t_{i, 0} = \theta^t + \lambda \Delta^t$, each participating client optimizes a local objective function.
%{The local objective function is defined as the sum of its local empirical loss function and a penalized loss function which is based on the local online model and the received server model:}
%
\iffalse
%
\begin{equation}
{\underset{\theta_{i,k}^{t+1}}{\operatorname{argmin}}}~ L_i(\theta_{i,k}^{t+1}) = f_i(\theta_{i,k}^{t+1}
) + \frac{\beta}{2}\|\theta_{i,k}^{t+1}-(\theta^t-\lambda\Delta^t)\|^2,
\label{eq:local_objective}
\end{equation}
%
\fi
%
\iffalse
\begin{equation}
%\theta_i^t = {\underset{\theta}{\operatorname{argmin}}}~f_i(\theta
%) + \frac{\beta}{2}\|\theta-(\theta^{t-1} + \lambda\Delta^{t-1})\|^2.
{\underset{\theta}{\operatorname{min}}}~\left\{ f_i(\theta) := \mathcal{L}_i(\theta
) + \frac{\beta}{2}\|\theta-(\theta^{t-1} + \lambda m^{t-1})\|^2\right\}.
\label{eq:local_objective}
\end{equation}
%
where $\beta$ controls the balance between the two terms.
After $K$ local updates, each client uploads their trained model $\theta_{i,K}^t$ to the server, and then the server constructs the next server model $\theta^{t}$ via a simple aggregation, \ie $\theta^t = \sum_{i \in \mathcal{S}_t} \omega_i \theta_{i, K}^t$.
\fi
\jkkim{Each client uploads their trained model $\theta_{i,K}^t$ to the server, and then the server constructs the next server model $\theta^{t}$ via a simple aggregation, \ie $\theta^t = \sum_{i \in \mathcal{S}_t} \omega_i \theta_{i, K}^t$.}
%as shown in~\cref{alg:proposed_method}.

\iffalse
%
\setlength{\textfloatsep}{10pt}
\begin{algorithm}[t]
\caption{FedAvg}
\label{alg:fedavg}
\SetAlgoLined

\KwIn{$\theta^0$, number of clients $N$, number of local iterations $K$, number of communication rounds $T$}
\For{$\text{each round}~t = 1, 2, \dots ,T$}{
Sample subset of clients $S_t \subseteq \{1, \dots, N\}$

Server sends $\theta^t$ to all clients $i \in S_t$ 

\For{$\text{each client}~ i \in S_t,~\textbf{in parallel}$}{
\For{$k = 1, \dots ,K$}{
{${\underset{\theta_{i,k}^t}{\operatorname{argmin}}}\ f_i(\theta_{i,k}^t
)$}
}
Client sends  $\theta_{i,K}^t$ back to the server}
\textbf{In server:}

\quad $\theta^{t+1}$ = $\frac{1}{|S_t|} \Sigma_{i \in S_t}\theta_{i,K}^{t}$
}
\textbf{Return} ~ $\theta^{t+1}$
\end{algorithm}
\fi
%


Let the local update of each participating client throughout $K$ iterations be $\Delta^t_i =\theta_{i,K}^{t}-(\theta^{t-1} + \lambda m^{t-1})$. 
The expected local updates of all participating clients is given by $\Delta^t = \sum_{i \in S_t} \omega_i \Delta^t_i = \theta^t - (\theta^{t-1} + \lambda m^{t-1})$.
%Let the average local update of all participating clients from the accelerated point by the global momentum be $\nabla (\theta^t) =-\frac{1}{|S_t|}\underset{i \in S_t}{\Sigma}(\theta_{i,K}^{t}-(\theta^{t-1}-\lambda\Delta^{t-1}))$. 
%Then the momentum $m_t$ can be computed by the exponential updates with the decay coefficient $\lambda$ as
Then, $m^t$ is given by the exponential updates with the decay coefficient $\lambda$ as
%
\begin{align}
%m_{t}&= \theta^{t}-\theta^{t-1} =\Delta^t + \lambda m_{t-1},
%m_{t}&= \Delta^t + \lambda m_{t-1}, \\
%           \\ &= -\frac{1}{|S_t|} \Sigma_{i \in S_t}\theta_{i,K}^{t} +\theta^{t-1}
%           \\ &= \nabla (\theta^t) - \theta^{t-1} + \lambda \Delta^{t-1} + \theta^{t-1}
%           \\&=\nabla(\theta^t) + \lambda \Delta^{t-1}
m^{t} = \theta^{t}-\theta^{t-1}  = \left[ \Delta^{t} + (\theta ^{t-1} + \lambda  m^{t-1}) \right]  - \theta^{t-1} %\\
           %&= \frac{1}{|S_t|} \Sigma_{i \in S_t}(\theta_{i,K}^{t+1} - (\theta^t+\lambda m_t)) + \lambda m_t \nonumber
           =\Delta^{t} + \lambda m^{t-1}.
\end{align}
%
Note that we use $m^t$ as the global momentum of the next round in our formulation.
%This means that $\Delta^t$ is an exponential moving average of the total local updates computed at the projected point with the decay coefficient $\lambda$.
%Although only a subset of clients participates in each communication round, $\Delta^t$ maintains past global gradient information, which serves as an approximation to the gradient of the global loss function $f(\theta)$.
%As illustrated in Figure~\ref{fig:gradient_acceleration}, we can view integrating $\lambda m_t$ to the global model $\theta^t$ at server-to-client transmission as taking a lookahead through the interim parameters where the accumulated global velocity will lead the global model.
As illustrated in Figure~\ref{fig:gradient_acceleration}, we take a lookahead by integrating $\lambda m^{t-1}$ to the previous global model $\theta^{t-1}$ and obtain the global model $\theta^t$ by further aggregating the local updates.
This anticipatory update in client side leads each client to find a local minima adjacent to the trajectory of the global gradients, which helps FedACG avoid inconsistent local updates. 
%Our approach has a similar motivation with meta-learning~\citep{finn2017model}, where a meta-learner learns initial parameters to accelerate the optimization for target tasks.
Our approach has a similar motivation with meta-learning~\citep{finn2017model}, where a meta-learner identifies the optimal point to facilitate the optimization of all target tasks.


\iffalse
%Since we define the server model update direction as $\Delta^{t+1} \equiv -(\theta^{t+1}-\theta^t)$,
the following Lemma~\ref{thm:delta_momentum} holds.
%
\begin{lemma}
\label{thm:delta_momentum}
Let the average local update of all participating clients computed in the server be $\nabla (\theta^t) =-\frac{1}{|S_t|}\underset{i \in S_t}{\Sigma}(\theta_{i,K}^{t}-(\theta^{t-1}-\lambda\Delta^{t-1}))$. Then $\Delta^t$ is exponentially updated as
\begin{equation}
    \Delta^{t} = \nabla(\theta^{t-1})+\lambda\Delta^{t-1}.
\end{equation}
\end{lemma} 
%
\iffalse
\begin{myproof}
\begin{align*}
\Delta^{t+1}&=-(\theta^{t+1}-\theta^{t})
           \\ &= -\frac{\tau}{|S_t|} \Sigma_{i \in S_t}\theta_{i,K}^{t} - (1-\tau) (\theta^t-\lambda\Delta^t)+\theta^t
           \\ &= -\frac{\tau}{|S_t|} \Sigma_{i \in S_t}(\theta_{i,K}^{t} - (\theta^t-\lambda\Delta^t)) + \lambda\Delta^t
           \\&=\tau\nabla(\theta^t) + \lambda \Delta^t
\end{align*}
\end{myproof} 
\fi
\begin{myproof}
\begin{align*}
\Delta^{t}&=-(\theta^{t}-\theta^{t-1})
           \\ &= -\frac{1}{|S_{t-1}|} \Sigma_{i \in S_{t-1}}\theta_{i,K}^{t-1} +\theta^{t-1}
           \\ &= \nabla (\theta^{t-1}) - \theta^{t-1} + \lambda \Delta^{t-1} + \theta^{t-1}
           \\&=\nabla(\theta^{t-1}) + \lambda \Delta^{t-1}
\end{align*}
\end{myproof}
%
Lemma~\ref{thm:delta_momentum} means that $\Delta^t$ is an exponential moving average of the total local updates computed at the projected point with the decay coefficient $\lambda$.
Although only a subset of clients participates in each communication round, $\Delta^t$ maintains past global gradient information, which serves as an approximation to the gradient of the global loss function $f(\theta)$.
\fi







\ghkim{
\subsection{Local objective function}}

In addition to the initial point acceleration for local training, 
we also augment the local loss function with a regularization term that penalizes the difference between the local online model and the accelerated model, which is given by
\begin{equation}
%\theta_i^t = {\underset{\theta}{\operatorname{argmin}}}~f_i(\theta
%) + \frac{\beta}{2}\|\theta-(\theta^{t-1} + \lambda\Delta^{t-1})\|^2.
{\underset{\theta^{t}_i}{\operatorname{min}}}~\left\{ \mathcal{F}_i(\theta^{t}_i) := \mathbb{E}_{(x, y) \sim \mathcal{D}_i} [f_i((x,y); \theta^t_i)] = \mathcal{L}_i(\theta^t_i
) + \frac{\beta}{2}\|\theta^t_i-(\theta^{t-1} + \lambda m^{t-1})\|^2\right\},
\label{eq:local_objective}
\end{equation}
%
where $\beta$ controls the balance between the two terms.
\jkkim{Then, the gradient of the local loss function is, }
\begin{equation}
   \nabla \mathcal{F}_i(\theta_i^t) =\mathcal{L}_i(\theta^t_i) + \beta\lambda m^{t-1} + \beta (\theta_i^t - \theta^{t-1}).
   \label{local_derivative_correction_term_prox}
\end{equation}
\jkkim{Note that we add $m^{t-1}$, delivered from the integrated message $\theta^{t-1} + \lambda m^{t-1}$, as a correction term to local gradient direction at every local step.
This term asymptotically aligns with the difference between global and local gradients, which further prevents each client from falling into its own biased minima.}
%%\vspace{0.5cm}

\begin{figure}[t]
\centering
\includegraphics[width=1\textwidth]{figures/test14.pdf}
\caption{An illustration of the proposed accelerated client gradient.
\iffalse\bhhan{We first accelerate the latest global model $\theta^{t-1}$ toward the server update direction $\lambda \Delta^{t-1}$.
Each participating client optimize its local loss starting from the accelerated point, which facilitates for a locally trained model $\theta_{i, K}^{i}$ to be adjacent to the trajectory of the global gradients.}\fi
%A server transmits the current model to the participating clients with the global momentum $\lambda m_{t-1}$.
\ghkim{We first partially update the previous global model in the direction of the global momentum (orange vector) and then make local updates (grey vector), resulting in the server model update (blue vector).
Through this anticipatory update, we adapt the individual local updates to the slope of the global loss function and speed up the convergence.}}
\iffalse
Each client starts its local updates from the momentum-integrated point, which facilitates for a locally trained model $\theta_{i, K}^{i}$ to be aligned with the trajectory of the global gradient.}
\fi
\label{fig:gradient_acceleration}
%\vspace{-0.1cm}
\end{figure}



\subsection{Discussion}
While our formulation has something common with the existing works that also address client heterogeneity by employing global gradient information for the local update, FedACG has the following major advantages.
%
%\paragraph{\revision{[No additional communication overhead]}}
First, contrary to \cite{karimireddy2019scaffold,xu2021fedcm,gao2022feddc}, the server and clients only communicate model parameters without imposing additional network overhead for transmitting gradients and other information; the server broadcasts $(\theta^{t-1} + \lambda m^{t-1})$ as a single message and each client sends $\theta_{i, K}^t$ to the server.
This is a critical benefit because the increase in communication cost challenges many realistic federated learning applications involving clients with limited network bandwidths.
%Also, FedAGM does not require the server to compute or maintain any historical information of the model, which leads to extra saving of computational cost in the server.
%
%\paragraph{\revision{[Do not keep local states, robust to partial participation scenario]}}
Second, FedACG is robust to the low participation rate of clients and allows new-arriving clients to join the training process immediately without a warmup phase because, unlike~\citet{karimireddy2019scaffold}, \citet{acar2021federated}, \citet{li2021model}, and \citet{gao2022feddc}, the clients are supposed to neither store their local states nor use them for model updates.
%Furthermore, the stored local states can easily get stale if only a small fraction of devices are active each round, and this will hurt the convergence of the algorithm.

\subsection{Convergence analysis of FedACG}

We now present the theoretical convergence rate of FedACG.
We first state two assumptions for the local loss functions $\ell_i(\theta)$, which are commonly used in several previous works on federated
optimization~\citep{karimireddy2019scaffold,reddi2021adaptive,xu2021fedcm,acar2021federated}.
First, the local function $\ell_i(\cdot)$ is assumed to be $L$-smooth for all $i \in \{1,\dots,N\}$, \ie
\begin{align}
\|\nabla \ell_i ({ x}) -\nabla \ell_i ({ y})\|\leq
L \|{ x} - { y}\|\ \ \forall { x}, { y}. 
\end{align}
%
Second, if we additionally assume the convexity of the functions $\{\ell_i(\cdot)\}_{i=1}^N$s, we have
\begin{align}
& \forall { x}, \ \ \ \ \ \ \  \frac{1}{2LN}\sum_{i=1}^{N} \|\nabla \ell_i ({x}) - \nabla \ell_i({x}_*)\|^2 \leq \ell({x})-\ell({x}_*) ~~\text{and}
\label{as:smooth_convex_min}\\
& \forall { x}, { y}, { z}, \  \left\langle \nabla \ell_i ({ x}), { z}- { y}\right\rangle \leq -\ell_i({ z}) +\ell_i({ y}) + \frac{L}{2} \|{ z} - { x}\|^2 ,
\label{as:smooth_convex_grad}
\end{align}
where $\ell({ x}) = \frac{1}{N} \sum_{i=1}^N \ell_i({ x})$ and $\nabla \ell({ x}_*)={ 0}$.
%
Based on the above assumptions, we derive the following asymptotic convergence bound of FedACG.
Note that we make no further assumptions such as a form of bounded variance and gradients used in~\citet{karimireddy2019scaffold}, \citet{reddi2021adaptive}, and \citet{xu2021fedcm}.
%
\begin{thm}
\label{thm:convex_main}
Assuming the convexity and $L$-smoothness of $\left\{\ell_{i}(\cdot)\right\}_{i=1}^{N}$, for $\frac{1}{2} < \lambda < 1$, Algorithm~\ref{alg:proposed_method} satisfies
\begin{align*}
\mathbb{E} & \left[\ell\left(\frac{1}{T} \sum_{t=1}^{T} \theta^{t-1}\right) - \ell\left({\theta}_{*} \right) \right] \\
 &\leq \frac{\sqrt{\lambda(1-\lambda)}}{T} \bigg( L \left\|\theta^{0}-{\theta}_{*}\right\|^{2}   
 +\frac{1}{LN} \sum_{i=1}^{N}\left\|\nabla \ell_{i}\left({\theta}_{i}^{0}\right)\right\|^{2}\bigg),
\end{align*}
%
where $\theta_{*}=\underset{\theta}{\arg \min }~ \ell(\theta)$ and $\theta^t=\frac{1}{|S_t|}\sum_{i \in {S_t}}\theta^t_i$.
\end{thm} 
%
Theorem~\ref{thm:convex_main} implies that, for convex and smooth local functions, the global objective function is expected to converge at a rate of $O\left(\frac{\sqrt{\lambda(1-\lambda)}}{T} \right)$.
This rate is the empirical loss averaged over all devices.
It further implies a higher value of $\lambda$ improves the convergence rate under the convex setting, which will be empirically verified in our experiments.
%In the experiments with practical datasets, we empirically show that a sufficiently large value of $\lambda$ is necessary for rapid convergence.
Please, refer to the supplementary document for the full proof.


\iffalse
The convergence rates of FedACG justify our claim that the proposed method is robust to the partial participation characteristics of federated learning.
Our result is free of the term $\frac{N}{S}$, which exists in the convergence rate of SCAFFOLD~\cite{karimireddy2019scaffold} and FedDyn~\cite{acar2021federated} as they require each client
to store local states.
This result is compatible with our
empirical findings that FedACG is robust under various heterogeneous clients and participation rates (Section~\ref{sec:experiment}).
\fi







\iffalse

as linear combination of averaged parameters received from clients $\frac{1}{|S_t|} \Sigma_{i \in S_t}\theta_{i,K}^{t}$ and the parameters distributed to clients.

For the regularization term, is to penalize 
in model communication process where
%the server projects the current model $\theta^t$ toward $\Delta^t$\jkkim{, which quantifies the direction for server model update} and sends the accelerated model $\theta^t - \lambda \Delta^t$ to the client.
The server aggregates the gradient information of previous active clients and sends the projected model $\theta^t - \lambda \Delta^t$ to the client instead of $\theta^t$.
\iffalse
\jkkim{The main modification in FedACG compared to FedAvg lies in the model that the server broadcasts to the client.
Unlike FedAvg passing the current global model($\theta^t)$, FedACG passes the accelerated global model($\theta^t-\lambda\Delta^t)$ where $\Delta^t$ is global update in the previous step and $\lambda$ is hyperparameter.
}
\fi
\jkkim{Starting with the projected parameter as an initial point, clients active in current round take local steps to minimize their local objective functions.}
After $K$ local updates, each client returns their parameters $\theta_{i,K}^t$. The server calculates the next model as linear combination of averaged parameters received from clients $\frac{1}{|S_t|} \Sigma_{i \in S_t}\theta_{i,K}^{t}$ and the parameters distributed to clients. 
We define server model update direction as $\Delta^{t+1}=-(\theta^{t+1}-\theta^t)$. 
Then the following~\cref{thm:delta_momentum} holds.





%\paragraph{\revision{[$\Delta^t$ is the momentum although not explicitly calculated]}}
Lemma 4.1 means that $\Delta^t$ is an exponential moving average of the total local updates computed at the projected point with the decay coefficient $\lambda$. 
Although only a subset of clients participate in each communication round, past local update information included in $\Delta^t$ is maintained.
Updating  the  current  model  using  it  can have the similar effect as increasing the participation rate which makes FedACG be robust to partial client participation in federated learning.
Therefore, since the momentum term $\Delta^t$ serves as an approximation to the gradient of the global loss function $f(\theta)$, we have the local update direction as follows:
\begin{equation}
\begin{aligned}
\nabla L_{i}(\theta_{i, k}^{t}) &=\alpha \nabla f_{i}(\theta_{i, k}^{t})+\beta(\theta_{i, k}^{t}-(\theta^{t}-\lambda \Delta^{t})) \\
&=\alpha \nabla f_{i}(\theta_{i, k}^{t}) +\beta \lambda \Delta^{t} +\beta (\theta_{i, k}^{t}-\theta^{t}) \\
&\approx(\alpha + \beta\lambda) \nabla f_{i}(\theta_{i, k}^{t}) +\beta \lambda (\nabla f(\theta) - \nabla f_{i}(\theta_{i, k}^{t})) \\
&\quad +\beta (\theta_{i, k}^{t}-\theta^{t})
\end{aligned}
\end{equation}

\iffalse
\paragraph{\revision{[Correct local update with global information $\Delta^t$ without communication cost]}}
\jkkim{
If each client knows the global update information and utilizes it for local update, it can be expected that client-drift due to data heterogeneity will be reduced. At first glance, this method seems to be possible only by communicating an additional message. However, the following lemma suggests that there is a detour.}
%
\begin{lemma}
\label{local correction}
Let the model that the $i$th client undergoes the $k$th local iteration be $\theta_{i,k}^t$. Then the local model is updated in the following way.
\begin{equation*}
    \theta_{i,k+1}^t=\theta_{i,k}^t-\eta_l\alpha \nabla f_i(\theta_{i,k}^t)  -\eta_l \beta(\theta_{i,k}^t-\theta^t)+ \eta_l\beta \lambda \Delta^t
\end{equation*}
\end{lemma} 
%
\begin{myproof}
Since $i$th client's local objective is \\
$L_i(\theta_{i,k}^t)=\alpha f_i(\theta_{i,k}^t
)+\frac{\beta}{2}\|\theta_{i,k}^t-(\theta^t+\lambda\Delta^t)\|^2$,\\
Its gradient is obtained as follows.
\begin{align*}
\nabla L_i(\theta_{i,k}^t) &=\alpha\nabla f_i(\theta_{i,k}^t
)+\beta(\theta_{i,k}^t-(\theta^t+\lambda\Delta^t))\\
&=\alpha\underbrace{\nabla f_i(\theta_{i,k}^t
)}_\text{local loss func}+\beta\underbrace{(\theta_{i,k}^t-\theta^t)}_\text{prox}-\underbrace{\beta\lambda\Delta^t}_\text{global momentum}
\end{align*}
\end{myproof}
\fi
This implies that FedACG has a correction toward global gradient direction with proximal term, which prevent each client from falling into its biased minima.

\jkkim{
\iffalse
This suggests a surprising fact. We can use global information for local update correction without communicating messages bigger than the model size.
\fi
\iffalse
This is effective in improving performance in a federated setting.
\fi
}
%\paragraph{\revision{[Why our method works or how our method handle client heterogeneity]}}
\iffalse
Moreover, $\Delta^t$ contains the update information of clients that participated in the past in the form of an exponential moving average, updating the current model using it \iffalse in this direction \fi can have the similar effect as increasing the participation rate.\fi
Furthermore, you can view adding $\lambda \Delta^t$ to current model $\theta^t$ when sending the model for local update as taking a lookahead through the interim parameters where the accumulated global velocity will lead the current model. 
If the velocity update leads to bad client loss, then the client will make a correction to minimize their loss properly.
This anticipatory update in client side allow the search to slow down when approaching the local optima and reduce the likelihood of going too far by the added global velocity, which helps FedACG avoid oscillations by client heterogeneity and achieves better performance.


\fi







==> sections/preliminary.tex <==
% !TEX root = ../main.tex

\section{Preliminaries}
\label{sec:preliminary}

%%\vspace{-0.4cm}

\subsection{Problem setting and notations}
%\paragraph{\revision{[Federated learning task]}}
%Given $N$ remotes clients for a task of federated learning,
%the goal of federated learning is to construct a single model that minimizes the following objective function.
\iffalse
\ghkim{In federated learning, we assume that there are $N$ remote clients which have their private data and perform individual computation and a central server which sends and aggregates messages from the clients.
Let $\ell_i(\theta)=\mathbb{E}_{(x, y) \sim \mathcal{D}_i}[\ell_i((x,y);\theta)]$ be the loss function of the $i$-th client from its private dataset $\mathcal{D}_i$, the goal of federated learning is to train a unified model $\theta$ that minimizes the average loss of all clients as follows:
}
\fi
In the federated learning setting, there are $N$ clients that optimize their local models based on the corresponding private datasets as well as a central server that broadcasts the global model and then aggregates messages from the clients.
Let $\mathcal{L}_i(\theta) := \mathbb{E}_{(x, y) \sim \mathcal{D}_i}[\ell_i((x,y);\theta)]$ be the loss function of the $i^\text{th}$ client with a local dataset denoted by $\mathcal{D}_i$.
Then, the goal of federated learning is to train a model that minimizes the average loss of all clients as follows:
%
\begin{equation}
\label{global_objective}
%    \underset{\theta}{\operatorname{min}}\left\{\ell(\theta) := \underset{i=1}{\overset{N}{\Sigma}} \frac{|\mathcal{D}_i|}{|\mathcal{D}|} \ell_i(\theta)\right\},
    \underset{\theta}{\operatorname{min}}\left\{\mathcal{L}(\theta) := \sum_{i=1}^N \omega_i \mathcal{L}_i(\theta)\right\},
\end{equation}
%
where $\theta$ is the parameter of the global model and $\omega_i$ is the normalized weight of the $i^\text{th}$ client determined by the size of the local dataset.
%where $f_i(\theta)=\mathbb{E}_{z \sim D_i}[f_i(\theta,z)]$ is the loss function of the $i$-th client.
%Note that clients may have heterogeneous data distributions, but communication of training data between clients and the central server is strictly prohibited due to privacy concerns. 
%\ghkim{Note that $\mathcal{D}_i$ may vary from client to client, which corresponds to data heterogeneity over clients}.
%\ghkim{Due to the privacy concern, any client is prohibited to communicate its raw data with others.}
%All the basic notations throughout this paper are listed in~\cref{tab:notation}.
We focus on the non-\textit{i.i.d} data setting where local datasets have heterogeneous distributions.
Note that the communication of training data between clients and the central server is strictly prohibited in principle due to privacy issues.

\iffalse
% The table contents will be modified.
\begin{table}[t]
\centering
\caption{Summary of notation used in the paper}
%\vspace{0.2cm}
\scalebox{0.85}{
\begin{tabular}{@{}cl@{}}
\hline
$N$ & total number of clients \\
$T$ & total number of communication rounds \\
$S_t$ & sampled number of clients in round $t$\\
$K$ & total number of local iterations \\
$i$ & client index \\
$D_i$ & data distribution of $i$th client \\
$\theta^t$ & shared model parameters in round $t$\\
 $\theta_{i,k}^t$ & local model of $i$th client in round $t$ and step $k$  \\
\hline
\end{tabular}}
\label{tab:notation}
%%\vspace{-0.1cm}
\end{table}
%\vspace{-0.1cm}
\fi


\subsection{FedAvg algorithm}
\label{sub:fedavg}
%\paragraph{\revision{[Fedavg and its difficulties encountered with non iid and partly participation ]}}
FedAvg~\citep{mcmahan2017communication} is a standard algorithm of federated learning, where the server simply aggregates all the participating client models to obtain the global one.
Specifically, in each round $t \in \{1,\dots,T\}$, a central server sends the global model $\theta^{t-1}$ 
\ghkim{to the subset of the clients $\mathcal{S}_i \subseteq \{1,\dots,N\}$. Each of client $i \in \mathcal{S}_i$ initializes its local model parameter $\theta^{t}_{i, 0}$ as $\theta^{t-1}$, \textit{i.e.}, $\theta_{i, 0} = \theta^{t-1}$, and performs $K$ steps of the gradient descent to minimize its local loss, which is given by
%
\begin{equation}
\label{local_update_fedavg}
   \theta^t_{i, k} = \theta^t_{i, k-1} - \eta g^t_{i, k-1},
\end{equation}
%
where $\theta^t_{i,k}$ denotes the online model parameter of client $i$ at $k^{\text{th}} \in \{1,\dots,K\}$ local steps, $g^t_{i,k} := \nabla \mathcal{L}_i(\theta^t_{i,k})$ is an unbiased stochastic gradient of $\mathcal{L}_i$, and $\eta$ represents a learning rate.}
\iffalse 
to each of the clients.
Each client initializes its local model parameter $\theta^{t}_{i, 0}$ as $\theta^{t-1}$, \textit{i.e.}, $\theta_{i, 0} = \theta^{t-1}$,  performs $K$ steps of the gradient descent optimization to minimize its local loss, and then returns the updated model parametrized by $\theta_{i,K}^t$ to the server. 
The local loss of FedAvg at the $k^\text{th}$ $ \in \{1, \dots, K\}$ local iteration is given by
%
\begin{equation}
\label{fedavg_loss}
   \mathcal{L}_i(\theta_{i,k}^t) = \mathbb{E}_{{(x,y)} \sim \mathcal{D}_i}[\ell_i((x,y) ; \theta_{i,k}^t)],
\end{equation}
%
where the cross-entropy loss is typically used for $\ell_i(\cdot ; \cdot)$.
\fi
\iffalse
The local model update is given by
%
\begin{equation}
\theta_{i,k}^t \leftarrow \theta_{i,k-1}^t - \eta \nabla \mathcal{L}_i,
\label{eq:local_update_fedavg}
\end{equation}
%
where $\eta$ is a hyperparameter.
%\input{algorithms/fedavg.tex}
%
\fi
%An updated global model for the next round training is obtained by averaging all the participating local models in the current communication round. 
The server obtains an updated global model for the next round training, $\theta^t$, by taking the expectation of all the participating local models in the current communication round, $t$. 

A large number of local updates in FedAvg before the aggregation in the server may reduce the communication cost for training.
However, in practice, it typically leads to the so-called client drift issue~\citep{karimireddy2019scaffold}, where the individual client updates are inconsistent due to significant overfitting on local client data. 
This phenomenon hampers FedAvg from converging to the global optimum over all clients.

